SMPLest-X: Ultimate Scaling for Expressive Human Pose and Shape Estimation

Expressive human pose and shape estimation (EHPS) unifies body, hands, and face motion capture with numerous applications. Despite encouraging progress, current state-of-the-art methods focus on training innovative architectural designs on confined datasets. In this work, we investigate the impact of scaling up EHPS towards a family of generalist foundation models. 1) For data scaling, we perform a systematic investigation on 40 EHPS datasets, encompassing a wide range of scenarios that a model trained on any single dataset cannot handle. More importantly, capitalizing on insights obtained from the extensive benchmarking process, we optimize our training scheme and select datasets that lead to a significant leap in EHPS capabilities. Ultimately, we achieve diminishing returns at 10M training instances from diverse data sources. 2) For model scaling, we take advantage of vision transformers (up to ViT-Huge as the backbone) to study the scaling law of model sizes in EHPS. To exclude the influence of algorithmic design, we base our experiments on two minimalist architectures: SMPLer-X, which consists of an intermediate step for hand and face localization, and SMPLest-X, an even simpler version that reduces the network to its bare essentials and highlights significant advances in the capture of articulated hands. With big data and the large model, the foundation models exhibit strong performance across diverse test benchmarks and excellent transferability to even unseen environments. Moreover, our finetuning strategy turns the generalist into specialist models, allowing them to achieve further performance boosts. Notably, our foundation models consistently deliver state-of-the-art results on seven benchmarks such as AGORA, UBody, EgoBody, and our proposed SynHand dataset for comprehensive hand evaluation. (Code is available at: https://github.com/wqyin/SMPLest-X).

==> figures/factors.tex <==
\begin{figure*}[t!]
  % \vspace{-3mm}
  \centering
  \includegraphics[width=\linewidth]{images/factors.pdf}
  \vspace{-5mm}
  \caption{\textbf{Analysis on dataset attributes.} We study the impact of a) the number of training instances, b) scenes, c) real or synthetic appearance, and d) annotation type, on dataset ranking in \Tab\ref{tab:single_datasets}.}
  \label{fig:factors}
  % \vspace{-0.5cm}
\end{figure*}


==> figures/full_visualization.tex <==

\begin{landscape}
\begin{figure}[h]
  \centering
  % \vspace{-5mm}
  \includegraphics[width=\linewidth]{images/full_visualization_h.pdf}
  % \vspace{-5mm}
  \caption{\textbf{More Visualization.} We compare \name-L32 with OSX~\cite{lin2023one} and Hand4Whole (H4W)~\cite{GyeongsikMoon2020hand4whole} (trained with the MSCOCO, MPII, and Human3.6M) in various scenarios.}
  \label{fig:full_visualization}
\end{figure}
\end{landscape}


==> figures/ranking_correlation.tex <==
% \begin{wrapfigure}{r}{0.4\textwidth}
\begin{figure}[h]
  \centering
  \includegraphics[width=0.8\linewidth]{images/ranking_correlation.pdf}
  \vspace{-0.3cm}
  \caption{\textbf{Correlation of benchmark datasets}. For each dataset, we train a model on its training set and evaluate its performance on the \textit{training} sets of seven benchmark datasets: 3DPW, AGORA, EgoBody (EgoSet), UBody, and ARCTIC and RenBody (High-resolution set). Datasets are then ranked by MPE. We study the correlation of benchmark datasets by their rankings among all datasets.}
  \label{fig:ranking_correlation}
\end{figure}
% \end{wrapfigure}


==> figures/visualization.tex <==
% \begin{wrapfigure}{r}{0.5\textwidth}
\begin{figure*}[t]
  \centering
  % \vspace{-2mm}
  \includegraphics[width=\linewidth]{images/visualization.pdf}
  % \vspace{-5mm}
  \caption{\textbf{Visualization.} We compare \name-L32 with OSX~\cite{lin2023one} and Hand4Whole (H4W)~\cite{GyeongsikMoon2020hand4whole} (trained with the MSCOCO, MPII, and Human3.6M) in various scenarios.}
  \label{fig:visualization}
\end{figure*}
% \end{wrapfigure}


==> sections/U_overview.tex <==
\section{Supp - Overview}
Due to space constraints in the main paper, We elaborate the following in \Supp: additional details of the \numdatasets datasets, including useful links to find their license statements and other ethics concerns in \Sec\ref{sec:supp:datasets}; additional details of the architecture, training and finetuning stages in \Sec\ref{sec:supp:foundation_model}; additional experiments and analyses on dataset distributions, benchmark correlations, finetuning strategies, in-domain training, and more visualization results in \Sec\ref{sec:supp:add_exp}; individual dataset ranking on the training sets of key evaluation benchmarks, complete results of the foundation models (including \name-H32) and the individual dataset benchmark in \Sec\ref{sec:supp:complete_results}.

==> tables/3dpw.tex <==
% \begin{wraptable}{r}{0.4\textwidth}
\begin{table}[t]
% \vspace{-0.7cm}
  \caption{\textbf{3DPW.} $\ddagger$ denotes the methods that use temporal (multi-frame) information. $\dagger$ and $\ast$ are finetuned on the 3DPW training set and trained on 3DPW training set only, respectively. Unit: \emph{mm}.}
  \label{tab:3dpw}
  \vspace{0mm}
  \centering
  % \resizebox{\linewidth}{!}{
  \begin{tabular}{lcccccc}
    \toprule    
    Method & MPJPE & PA-MPJPE  \\
    \midrule
    \multicolumn{3}{c}{Body-only (SMPL) Methods} \\
    \midrule
    HybrIK~\cite{li2020hybrik} & 71.6 & 41.8 \\
    CLIFF~\cite{li2022cliff} & 68.0 & 43.0 \\
    HMR 2.0a & 70.0 & 44.5 \\
    Multi-HMR & 69.5 & 46.9 \\
    WHAM-B$\ddagger$ & 56.9 & 35.7 \\
    NLF-L & 54.9 & 33.6 \\

    \midrule
    \multicolumn{3}{c}{Whole-Body (SMPL-X) Methods} \\
    \midrule
    Hand4Whole~\cite{GyeongsikMoon2020hand4whole} & 86.6 & 54.4\\
    ExPose~\cite{PavlakosGeorgios2020expose} & 93.4 & 60.7 \\
    OSX~\cite{lin2023one}$\dagger$ & 86.2 & 60.6 \\
    \name-B1$\ast$ & 95.6 & 67.6 \\
    \name-L20 & 78.3 & 52.1 \\
    \name-L32 & \textbf{75.2} & \textbf{50.5} \\
    \name-L20$\dagger$ & \underline{76.8} & \underline{51.5} \\

    \bottomrule
    \end{tabular}
  % \vspace{-10mm}
% \end{wraptable}
\end{table}

==> tables/finetune_network.tex <==
\begin{table*}
  \caption{\textbf{Finetuning strategy}. We study the different finetuning strategies by freezing the parameters in different parts of the network. Models are tested on UBody test set, and $\dagger$ denotes the models that are finetuned on UBody train set. }
  \label{tab:finetune_network}
  \centering
  \resizebox{0.8\textwidth}{!}{
  \begin{tabular}{lcccccccc}
    \toprule
    & & & \multicolumn{3}{c}{PA-PVE (\textit{mm})} &
    \multicolumn{3}{c}{PVE (\textit{mm})} \\
    
    \cmidrule(lr){4-6} \cmidrule(lr){7-9}
    
    Method & Finetune & \#Param. &
    All & Hands & Face &
    All & Hands & Face \\
    
    \midrule
    \name-H32 & - & 662M &
    29.9 & 9.8 & 2.6 & 54.5 & 36.4 & 20.6 \\
    
    \name-H32$\dagger$ & Full network & 662M & 
    27.8 & 9.0 & 2.3 & 51.3 & 32.6 & 19.1 \\
    
    \name-H32$\dagger$ & Neck+Head & 31M & 
    27.8 & 9.0 & 2.3 & 51.1 & 32.5 & 19.1 \\
    
    \name-H32$\dagger$ & Head & 5M &
    29.9 & 9.7 & 2.6 & 54.2 & 35.9 & 20.6 \\
    
    \bottomrule
  \end{tabular}}
\end{table*}


==> tables/full_results.tex <==


\begin{sidewaystable}
    \centering
    \caption{Complete results of individual dataset benchmark with the same setting as Table 1 in the main paper. We train a model for each dataset on its training set and evaluate its performance on the \textit{training} sets of six benchmarks. Top-1 values are bolded, and the rest of the Top-5 are underlined. Unit: mm.}
    \label{tab:full_res}
    \resizebox{1.05\textwidth}{!}{
    \begin{tabular}{l|cccccc|cccccccc|cccccccc|cc|cccccccc|cccccccc}
    
    \toprule 
    & \multicolumn{6}{c}{AGORA~\cite{patel2021agora}} & \multicolumn{8}{c}{UBody~\cite{lin2023one}} & 
    \multicolumn{8}{c}{EgoBody~\cite{zhang2022egobody}} & \multicolumn{2}{c}{3DPW~\cite{von2018recovering}} & \multicolumn{8}{c}{ARCTIC~\cite{fan2023arctic}} & \multicolumn{8}{c}{RenBody~\cite{renbody} } \\
    \cmidrule(lr){2-7} \cmidrule(lr){8-15} \cmidrule(lr){16-23} \cmidrule(lr){24-25} \cmidrule(lr){26-33} \cmidrule(lr){34-41}
    
    & \multicolumn{3}{c}{PA-PVE$\downarrow$} & \multicolumn{3}{c}{PVE$\downarrow$} & 
    \multicolumn{3}{c}{PA-PVE$\downarrow$} & \multicolumn{3}{c}{PVE$\downarrow$} & \multicolumn{2}{c}{PA-MPJPE$\downarrow$} &
    \multicolumn{3}{c}{PA-PVE$\downarrow$} & \multicolumn{3}{c}{PVE$\downarrow$} & \multicolumn{2}{c}{PA-MPJPE$\downarrow$} &
    \multicolumn{2}{c}{PA-MPJPE$\downarrow$} &
    \multicolumn{3}{c}{PA-PVE$\downarrow$} & \multicolumn{3}{c}{PVE$\downarrow$} & \multicolumn{2}{c}{PA-MPJPE$\downarrow$} &
    \multicolumn{3}{c}{PA-PVE$\downarrow$} & \multicolumn{3}{c}{PVE$\downarrow$} & \multicolumn{2}{c}{PA-MPJPE$\downarrow$} \\
    \cmidrule(lr){2-4} \cmidrule(lr){5-7} 
    \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-15} 
    \cmidrule(lr){16-18} \cmidrule(lr){19-21} \cmidrule(lr){22-23}
    \cmidrule(lr){24-25} 
    \cmidrule(lr){26-28} \cmidrule(lr){29-31} \cmidrule(lr){32-33}
    \cmidrule(lr){34-36} \cmidrule(lr){37-39} \cmidrule(lr){40-41}   
        
      Dataset &  All &  Hand &  Face &  All &  Hand &  Face &  All &  Hand &  Face &  All &  Hand &  Face &  Body &  Hand &  All &  Hand &  Face &  All &  Hand &  Face &  Body &  Hand &  Body &  Body &  All &  Hand &  Face &  All &  Hand &  Face &  Body &  Hand &  All &  Hand &  Face &  All &  Hand &  Face &  Body &  Hand \\

      \midrule
        MSCOCO~\cite{lin2014microsoft} & 75.7 & \underline{12.0} & \underline{5.1} & 174.4 & 76.5 & 79.1 & \underline{42.2} & \underline{10.3} & \underline{2.9} & \underline{94.5} & \underline{47.3} & \underline{28.2} & \underline{49.3} & \underline{10.6} & \underline{53.4} & 10.4 & \underline{3.7} & \underline{114.4} & \underline{49.8} & \underline{42.7} & \underline{62.3} & 10.7 & 102.7 & 69.3 & \underline{62.3} & 17.2 & 4.9 & \underline{122.7} & \underline{54.4} & 56.8 & \underline{69.0} & 17.0 & 59.5 & \underline{9.4} & \underline{3.7} & 104.3 & 52.5 & 49.7 & 60.8 & \underline{9.5} \\
        
        BEDLAM~\cite{black2023bedlam} & \underline{74.8} & \underline{12.1} & \underline{5.6} & \underline{159.0} & \underline{72.2} & \underline{67.8} & 64.9 & \underline{10.8} & 5.0 & 133.6 & \underline{60.8} & \underline{39.4}& 85.3 & \underline{11.0} & 59.6 & \underline{9.7} & 4.8 & 110.3 & \underline{47.7} & \underline{42.4} & \underline{79.0} & \underline{9.9} & {103.0} & 78.1 & \underline{65.4} & 18.5 & \underline{3.5} & \underline{103.6} & 58.5 & \underline{39.9} & 77.7 & 18.3 & 57.9 & 10.2 & 4.4 & \underline{91.0} & \underline{49.2} & \underline{42.4} & 68.8 & 10.2 \\
        
        GTA-Human~\cite{cai2021playing} & \underline{69.1} & 15.6 & 6.1 & \underline{153.4} & \underline{71.4} & \underline{69.5} & 66.3 & 18.9 & 4.9 & 136.5 & 67.1 & 52.0 & 84.9 & 19.1 & \underline{57.3} & 17.6 & 4.6 & 124.4 & 52.6 & 54.0 & \underline{66.5} & 18.1 & \textbf{93.5} & \textbf{59.4} & \underline{61.0} & \underline{15.6} & 5.6 & 132.8 & \underline{50.8} & 70.7 & \underline{66.7} & \underline{15.6} & \underline{52.6} & 12.8 & 4.5 & 107.6 & \underline{48.6} & 52.5 & \underline{57.1} & 13.0 \\
        
        SPEC~\cite{kocabas2021spec} & \underline{73.7} & 20.2 & 30.1 & \underline{137.7} & \underline{64.9} & 78.0 & 68.3 & 21.0 & 28.8 & 129.6 & \underline{59.9} & 59.5 & 78.5 & 19.4 & 65.6 & 19.6 & 28.8 & 126.7 & \underline{49.1} & 62.2 & 69.2 & 18.0 & 114.2 & 68.0 & 70.4 & 23.5 & 30.1 & 137.5 & \underline{54.1} & 56.3 & \underline{70.6} & 22.6 & 65.2 & 17.9 & 29.9 & 112.5 & \underline{48.7} & 55.2 & 64.1 & 16.1 \\
        
        AGORA~\cite{patel2021agora} & \textbf{40.3} & \textbf{7.6} & \textbf{4.0} & \textbf{83.4} & \textbf{42.1} & \textbf{38.5} & 68.1 & 11.4 & 4.6 & 135.1 & 64.9 & 51.7 & 91.5 & 11.6 & 66.4 & 10.9 & \underline{4.1} & 149.0 & 61.2 & 61.1 & 78.9 & 11.2 & 111.4 & 65.6 & \underline{69.2} & \underline{16.6} & \textbf{3.1} & 143.1 & 57.3 & 57.7 & 77.5 & 16.5 & \underline{51.4} & 10.6 & \underline{3.9} & 126.8 & 53.1 & 50.8 & \underline{52.8} & 10.7 \\
        
        SynBody~\cite{yang2023synbody} & \underline{74.1} & 20.0 & \underline{5.6} & \underline{155.2} & \underline{72.6} & \underline{69.4} & 75.5 & 21.1 & 5.2 & 141.6 & 73.2 & 49.9 & 87.1 & 22.1 & 79.1 & 23.2 & 4.9 & 137.0 & 65.9 & 59.5 & 91.2 & 24.5 & 99.4 & 69.6 & 80.7 & \underline{15.7} & \textbf{3.1} & 155.6 & 59.0 & 72.0 & 87.8 & \underline{16.0} & \underline{55.1} & 18.2 & 4.5 & \underline{91.5} & 51.3 & 46.2 & 60.2 & 19.0 \\
        
        PoseTrack~\cite{andriluka2018posetrack} & 86.7 & 21.0 & 16.3 & 177.9 & 89.0 & 88.8 & \underline{56.8} & 21.0 & 16.7 & \underline{119.2} & 66.6 & 55.7 & \underline{62.2} & 19.6 & 64.4 & 18.6 & 15.4 & 122.9 & 63.0 & 61.5 & 68.8 & 17.2 & 115.9 & 81.5 & 71.1 & 24.8 & 16.8 & 127.7 & 66.7 & 57.0 & 81.3 & 23.8 & 74.5 & 20.9 & 15.7 & 123.5 & 73.0 & 59.4 & 76.8 & 19.4 \\
        
        Egobody-EgoSet~\cite{zhang2022egobody} & 92.6 & 12.6 & \underline{5.6} & 188.0 & 93.9 & 86.3 & \underline{61.7} & 11.6 & \underline{4.1}& \underline{117.0} & \underline{60.4} & \underline{36.7} & \underline{73.7} & 11.7 & \textbf{37.1} & \textbf{7.8} & \textbf{2.7} & \textbf{47.7} & \textbf{34.6} & \textbf{20.9} & \textbf{46.0} & \textbf{7.9}  & 113.6 & 83.8 & 72.0 & 19.4 & 4.7 & \underline{119.0} & 56.7 & \underline{51.2} & 84.1 & 19.3 & 73.5 & 11.0 & 4.2 & 125.9 & 70.8 & 49.6 & 84.4 & 11.0 \\
        
        PROX~\cite{hassan2019resolving} & 86.1 & \underline{11.9} & \underline{5.6} & 189.1 & 86.2 & 83.5 & \underline{59.4} & \underline{10.5} & 4.6 & 161.1 & 66.4 & 53.9 & 75.8 & \underline{10.7} & \underline{55.6} & 10.1 & \underline{4.2} & \underline{116.9} & 53.5 & 51.7 & \underline{65.5} & 10.3 & 104.3 & 72.8 & \underline{61.0} & 17.6 & \underline{3.4} & 140.2 & 57.3 & \underline{49.8} & \underline{66.2} & 17.4 & 64.0 & 10.3 & 4.3 & 108.3 & 60.1 & 45.3 & 68.6 & 10.3 \\
        
        CrowdPose~\cite{li2019crowdpose} & 94.0 & 21.7 & 19.8 & 189.7 & 85.3 & 91.4 & 86.9 & 21.8 & 21.4 & 132.2 & 73.1 & 50.9 & 137.4 & 19.9 & 83.3 & 18.7 & 19.7 & 139.8 & 64.3 & 54.6 & 104.9 & 16.8 & 113.7 & 80.6 & 88.1 & 25.1 & 20.8 & 162.7 & 68.2 & 67.0 & 112.5 & 23.9 & 76.4 & 21.3 & 19.2 & 141.2 & 65.5 & 63.1 & 85.0 & 19.5 \\
        
        EgoBody-MVSet~\cite{zhang2022egobody} & 79.6 & \underline{12.4} & \underline{5.0} & 176.5 & {81.7} & \underline{76.8} & 67.2 & 11.4 & \underline{4.3} & 191.4 & 68.0 & 52.9 & 93.2 & 11.6 & \underline{55.7} & \underline{9.5} & \underline{3.5} & \underline{113.3} & \underline{49.4} & \underline{44.9} & 69.3 & \underline{9.6} & \underline{96.6} & 67.6 & 72.8 & 19.4 & \underline{3.7} & 138.8 & 59.6 & \underline{49.8} & 87.1 & 19.3 & 57.7 & 11.2 & \underline{3.5} & 101.9 & 55.8 & \underline{42.5} & 66.1 & 11.2 \\
        
        MPI-INF-3DHP~\cite{mehta2017monocular} & 91.0 & \underline{11.9} & 6.2 & 199.1 & 89.9 & 93.8 & 79.0 & \underline{10.4} & 6.1 & 147.0 & 73.7 & 75.3 & 99.1 & \underline{10.5} & 66.8 & \underline{9.9} & 5.5 & 128.7 & 56.9 & 63.5 & 79.5 &\underline{10.1} & 105.8 & \underline{65.1} & 69.8 & 17.2 & \underline{3.9} & 152.7 & 61.6 & 69.4 & 83.1 & 16.9 & 59.1 & 10.4 & 4.8 & 127.8 & 60.1 & 68.3 & 60.7 & 10.3 \\
        
        UBody~\cite{lin2023one} & 96.1 & 14.2 & 5.8 & 194.4 & 87.1 & 99.4 & \textbf{31.9} & \textbf{9.6} & \textbf{2.7} & \textbf{43.7} & \textbf{39.3} & \textbf{19.1} & \textbf{37.7} & \textbf{9.8} & 64.0 & 11.9 & 4.4 & 123.2 & 52.5 & \underline{44.7} & 74.2 & 12.3 & 131.3 & 98.6 & 70.3 & 17.2 & 5.7 & 157.2 & 56.1 & 78.7 & 83.2 & 17.1 & 87.9 & \underline{9.2} & 4.6 & 145.1 & 63.3 & 79.6 & 103.3 & \underline{9.3} \\
        
        RICH~\cite{huang2022capturing} & 93.3 & \underline{12.1} & 6.0 & 182.7 & 83.7 & 79.3 & 77.4 & 11.2 & \underline{4.5} & 159.4 & 67.9 & 43.5 & 100.0 & 11.4 & 85.8 & \underline{9.7} & 4.9 & 138.9 & 56.0 & 47.6 & 109.4 & \underline{10.0} & 123.2 & 93.2 & 79.6 & 18.6 & 4.6 & 142.6 & 58.7 & \underline{45.3} & 104.7 & 18.5 & 74.3 & \underline{9.7} & 4.8 & 104.3 & 56.7 & \underline{43.3} & 87.4 & \underline{9.8} \\
        
        MuCo-3DHP~\cite{Mehta2018SingleShotM3} & 106.5 & 23.5 & 69.7 & 205.7 & 86.1 & 129.4 & 104.4 & 22.4 & 70.7 & 202.6 & 77.7 & 113.8 & 88.8 & 20.6 & 90.4 & 20.2 & 69.7 & 162.8 & 65.3 & 108.8 & \underline{67.8} & 18.4 & 104.4 & \underline{60.3} & 95.6 & 25.7 & 68.6 & 166.4 & 69.2 & 114.2 & 76.2 & 24.5 & 86.8 & 21.6 & 69.4 & 156.9 & 67.5 & 115.6 & \underline{56.1} & 19.8 \\
        
        InstaVariety~\cite{kanazawa2019learning} & 148.0 & 20.3 & 73.3 & 230.3 & 92.5 & 204.8 & 130.2 & 20.2 & 75.1 & 181.2 & 68.9 & 186.9 & \underline{66.9} & 19.0 & 133.3 & 17.8 & 74.1 & 172.6 & 68.2 & 182.9 & 74.3 & 16.6 & \underline{97.8} & \underline{62.5} & 139.5 & 24.8 & 73.1 & 189.1 & 69.1 & 186.9 & 81.7 & 24.0 & 134.7 & 20.5 & 73.5 & 165.7 & 74.1 & 184.4 & 70.1 & 19.3 \\
        
        BEHAVE~\cite{bhatnagar2022behave} & 86.1 & 15.2 & 13.7 & 182.8 & 84.2 & 86.3 & 83.5 & 15.5 & 12.8 & 212.7 & 80.4 & 54.7 & 115.2 & 16.0 & 133.3 & 17.8 & 74.1 & 172.6 & 68.2 & 182.9 & 74.3 & 16.6 & 116.1 & 71.2 & 91.2 & \textbf{14.4} & 14.0 & 167.1 & 56.8 & 60.8 & 115.8 & \textbf{14.3} & 66.6 & 11.7 & 13.1 & 127.1 & 63.9 & 54.4 & 71.5 & 12.1 \\
        
        UP3D~\cite{lassner2017unite} & 95.3 & 21.7 & 18.1 & 228.3 & 97.8 & 97.8 & 80.0 & 20.5 & 19.0 & 181.4 & 89.6 & 58.0 & 97.8 & 18.5 & 82.6 & 18.3 & 17.8 & 160.3 & 74.9 & 59.2 & 95.2 & 16.4 & 142.4 & 96.6 & 91.2 & 24.4 & 18.1 & 197.3 & 77.7 & 80.2 & 113.6 & 23.0 & 84.6 & 20.5 & 18.1 & 173.5 & 79.7 & 73.0 & 98.4 & 18.7 \\
        
        ARCTIC~\cite{fan2023arctic} & 117.8 & 15.0 & 6.9 & 250.8 & 108.9 & 123.7 & 73.7 & 13.3 & 6.4 & 152.3 & 78.3 & 52.3 & 79.2 & 13.4 & 78.5 & 11.5 & 6.1 & 135.8 & 60.1 & 49.2 & 88.6 & 11.5 & 174.6 & 102.4 & \textbf{44.6} & 19.1 & \underline{3.4} & \textbf{71.2} & \textbf{42.5} & \textbf{37.2} & \textbf{47.1} & 19.1 & 87.1 & 13.2 & 5.8 & 172.7 & 87.5 & 93.7 & 88.9 & 13.0 \\
        
        3DPW~\cite{von2018recovering} & 88.9 & 33.7 & 17.6 & 190.8 & 89.3 & 91.9 & 82.9 & 35.2 & 14.6 & 218.2 & 88.2 & 56.2 & 106.9 & 32.1 & 75.1 & 35.9 & 15.1 & 143.6 & 73.6 & 60.0 & 82.9 & 32.9 & \underline{95.4} & 67.4 & 96.7 & 31.8 & 17.0 & 154.7 & 65.3 & 71.1 & 120.5 & 29.6 & 67.6 & 33.3 & 17.8 & 107.3 & 73.9 & 60.4 & 60.9 & 30.2 \\
        
        OCHuman~\cite{zhang2019pose2seg} & 109.0 & 25.2 & 18.4 & 216.1 & 95.6 & 110.4 & 89.3 & 22.7 & 18.5 & 199.3 & 83.4 & 63.7 & 122.1 & 20.8 & 98.4 & 20.4 & 16.8 & 165.9 & 71.9 & 64.6 & 115.9 & 18.7 & 157.0 & 112.3 & 101.6 & 25.0 & 17.7 & 191.3 & 68.2 & 71.7 & 124.5 & 23.8 & 105.2 & 23.7 & 17.3 & 172.8 & 83.0 & 85.5 & 114.2 & 21.6 \\
        
        CHI3D~\cite{fieraru2020three} & 75.4 & 18.6 & \underline{5.7} & 192.2 & 78.2 & 87.1 & 82.7 & 19.8 & 5.2 & 267.6 & 99.5 & 58.9 & 89.6 & 20.6 & 77.2 & 21.8 & 5.1 & 180.3 & 78.1 & 60.7 & 85.4 & 22.9 & 103.7 & \underline{64.9} & 81.5 & \underline{15.6} & 4.4 & 168.0 & 69.5 & 53.9 & 86.5 & \underline{15.7} & \underline{52.3} & 16.5 & \underline{4.0} & \underline{98.9} & 54.0 & 45.2 & \underline{53.0} & 17.1 \\
        
        RenBody-HiRes~\cite{renbody} & 90.1 & 14.7 & 6.1 & 210.2 & 80.5 & 111.4 & 79.5 & 12.9 & 5.0 & 267.3 & 66.1 & 77.9 & 106.1 & 13.3 & 76.4 & 12.4 & 4.6 & 181.9 & 57.0 & 67.3 & 96.2 & 12.8 & 125.4 & 77.3 & 72.6 & 17.5 & 5.0 & 161.9 & \underline{53.5} & 52.9 & 84.9 & 17.5 & \textbf{33.1} & \textbf{5.6} & \textbf{2.6} & \textbf{41.7} & \textbf{28.8} & \textbf{21.6} & \textbf{39.2} & \textbf{5.7} \\
        
        MTP~\cite{muller2021self} & 107.3 & 12.5 & 7.3 & 229.7 & 104.6 & 113.7 & 89.7 & 11.2 & 7.1 & 206.3 & 83.0 & 50.8 & 116.9 & 11.2 & 99.5 & \underline{10.0} & 6.7 & 169.4 & 65.9 & 56.3 & 135.2 & 10.1 & 181.0 & 116.8 & 109.9 & 17.8 & 6.3 & 184.7 & 66.3 & 76.8 & 151.5 & 17.6 & 100.5 & 10.9 & 6.2 & 177.3 & 87.4 & 95.9 & 120.3 & 10.8 \\
        
        HumanSC3D~\cite{fieraru2021learning} & 94.4 & 18.4 & 6.4 & 201.3 & 84.8 & 90.6 & 95.7 & 19.1 & 6.5 & 310.2 & 74.9 & 91.1 & 145.0 & 19.7 & 84.7 & 21.2 & 5.6 & 180.5 & 66.8 & 66.1 & 113.2 & 22.1 & \underline{99.2} & 70.6 & 94.5 & \underline{15.9} & 6.3 & 177.4 & 61.5 & 56.2 & 118.9 & \underline{16.0}& 60.8 & 16.9 & 4.8 & 114.5 & 60.1 & 52.8 & 60.8 & 17.4 \\
        
        RenBody~\cite{renbody} & 90.9 & 14.3 & 6.8 & 204.1 & 78.9 & 92.9 & 86.9 & 12.5 & 6.0 & 267.3 & 82.3 & 66.3 & 107.7 & 12.8 & 89.1 & 12.2 & 5.9 & 219.7 & 66.2 & 70.7 & 108.4 & 12.6 & 131.0 & 92.8 & 85.6 & 17.5 & 7.1 & 177.7 & 57.5 & 54.9 & 98.7 & 17.4 & 58.1 & \underline{6.6} & 5.1 & \underline{77.4} & \underline{38.7} & \underline{33.4} & 72.1 & \underline{6.7} \\
        
        FIT3D~\cite{fieraru2021aifit} & 114.4 & 19.3 & 5.9 & 253.3 & 93.1 & 106.5 & 100.9 & 19.5 & 5.8 & 299.3 & 88.1 & 62.0 & 129.3 & 20.1 & 90.6 & 21.6 & 5.3 & 201.7 & 68.4 & 64.6 & 110.0 & 22.4 & 111.9 & 75.9 & 95.4 & 15.9 & 5.5 & 237.6 & 65.6 & 83.5 & 108.0 & \underline{15.9} & 72.2 & 17.4 & 4.4 & 140.1 & 64.1 & 63.0 & 75.2 & 17.7 \\
        
        MPII~\cite{andriluka14cvpr}  & 155.5 & 33.6 & 16.3 & 252.5 & 107.6 & 131.0 & 120.5 & 34.9 & 16.2 & 227.8 & 91.5 & 90.7 & 161.6 & 31.7 & 129.1 & 35.7 & 16.3 & 211.8 & 90.9 & 96.8 & 148.9 & 32.6 & 183.3 & 147.0 & 129.1 & 31.6 & 15.8 & 232.0 & 83.4 & 138.8 & 149.3 & 29.4 & 142.7 & 33.2 & 15.6 & 205.6 & 102.5 & 121.8 & 157.7 & 30.0 \\
        
        Talkshow~\cite{yi2023generating} & 109.6 & 13.7 & 6.8 & 281.3 & 128.4 & 132.0 & 72.3 & 12.3 & 4.6 & \underline{125.6} & 66.6 & \underline{42.1} & 106.0 & 12.2 & 94.2 & 11.1 & 5.3 & 188.4 & 76.9 & 53.2 & 115.2 & 11.2 & 283.1 & 140.9 & 128.7 & 18.8 & 6.6 & 271.5 & 82.2 & 89.1 & 164.4 & 18.4 & 105.7 & 13.6 & 5.0 & 255.3 & 116.8 & 115.7 & 125.6 & 13.3 \\
        
        Human3.6M~\cite{ionescu2013human3} & 108.5 & 33.6 & 20.1 & 236.2 & 104.6 & 112.1 & 98.9 & 35.0 & 21.1 & 321.7 & 99.4 & 99.9 & 138.2 & 31.8 & 98.4 & 35.8 & 21.4 & 215.3 & 101.6 & 85.1 & 120.8 & 32.7 & 116.7 & 74.2 & 98.6 & 31.6 & 20.5 & 229.3 & 91.7 & 74.3 & 113.1 & 29.4 & 78.2 & 33.1 & 20.2 & 136.5 & 99.5 & 73.0 & 69.9 & 30.0 \\
        
        SSP3D~\cite{Sengupta2020SyntheticTF} & 165.2 & 33.9 & 19.4 & 261.8 & 111.4 & 187.3 & 151.0 & 35.4 & 18.2 & 244.0 & 125.4 & 197.6 & 180.1 & 32.1 & 165.4 & 36.2 & 18.2 & 238.5 & 108.9 & 211.8 & 181.1 & 32.9 & 242.9 & 167.8 & 165.7 & 31.6 & 17.8 & 297.1 & 101.8 & 236.9 & 182.8 & 29.2 & 165.5 & 33.3 & 18.6 & 245.3 & 108.7 & 187.9 & 173.1 & 30.0 \\
        
        LSPET~\cite{Johnson2011LearningEH} & 207.0 & 36.9 & 23.1 & 345.2 & 107.0 & 207.6 & 188.2 & 38.4 & 23.3 & 322.5 & 116.9 & 145.4 & 257.1 & 33.6 & 209.0 & 40.3 & 23.2 & 322.4 & 103.8 & 148.3 & 273.9 & 35.7 & 353.6 & 271.1 & 238.0 & 32.2 & 23.7 & 372.5 & 96.9 & 176.9 & 330.4 & 28.4 & 223.1 & 35.6 & 22.9 & 343.9 & 108.3 & 197.8 & 303.5 & 30.5 \\
        
      \bottomrule
    \end{tabular}}
\end{sidewaystable}


==> tables/speed_test.tex <==
\begin{table}[t]
% \vspace{-0.7cm}
  \caption{\textbf{Inference Speed.} Unit: \emph{mm}.}
  \label{tab:scale_cnn}
  \vspace{0mm}
  \centering
  % \resizebox{\linewidth}{!}{
  \begin{tabular}{lc}
    \toprule    
    Model &  Small & Base & Large & Huge \\
    \midrule
    OSX~\cite{lin2023one} & 12.17
    \name-single-frame & 36.17 & 33.09 & 24.44 & 17.47 \\

    \bottomrule
    \end{tabular}
  % \vspace{-10mm}
% \end{wraptable}
\end{table}
